Learning Depthwise Separable Graph Convolution from Data Manifold

Convolution Neural Network (CNN) has gained tremendous success in computer vision tasks with its outstanding ability to capture the local latent features. Recently, there has been an increasing interest in extending convolution operations to the non-Euclidean geometry. Although various types of convolution operations have been proposed for graphs or manifolds, their connections with traditional convolution over grid-structured data are not well-understood. In this paper, we show that depthwise separable convolution can be successfully generalized for the unification of both graph-based and grid-based convolution methods. Based on this insight we propose a novel Depthwise Separable Graph Convolution (DSGC) approach which is compatible with the tradition convolution network and subsumes existing convolution methods as special cases. It is equipped with the combined strengths in model expressiveness, compatibility (relatively small number of parameters), modularity and computational efficiency in training. Extensive experiments show the outstanding performance of DSGC in comparison with strong baselines on multi-domain benchmark datasets.

==> src/simulation.tex <==

\begin{figure*}[!th]
\centering
\begin{subfigure}{.25\linewidth}
  \includegraphics[width=\linewidth]{fig/shift.pdf}
  \caption{Shift}
\end{subfigure}
\hspace{0.35cm}
\begin{subfigure}{.25\linewidth}
  \includegraphics[width=\linewidth]{fig/rotate.pdf}
  \caption{Rotation}
\end{subfigure}
\hspace{0.35cm}
\begin{subfigure}{.25\linewidth}
  \includegraphics[width=\linewidth]{fig/flip.pdf}
  \caption{Left-Right Flip}
\end{subfigure}
\caption{Toy examples visualizing 3 graph operations: Shift, Rotation and Left-Right Flipping.}
\label{fig:sim}
\end{figure*}
\begin{figure*}[!th]
\centering
\begin{subfigure}{.275\linewidth}
  \includegraphics[width=\linewidth]{fig/shift-result.png}
  \caption{Shift}
\end{subfigure}
\hspace{0.3cm}
\begin{subfigure}{.275\linewidth}
  \includegraphics[width=\linewidth]{fig/rotation-result.png}
  \caption{Rotation}
\end{subfigure}
\hspace{0.3cm}
\begin{subfigure}{.275\linewidth}
  \includegraphics[width=\linewidth]{fig/flip-result.png}
  \caption{Left-Right Flip}
\end{subfigure}
\caption{Binary Cross Entropy (BCE) loss vs. training epoch for DSGC and GC on simulated data}
\label{fig:sim-result}
\end{figure*}

\subsection{Simulation-based Analysis}
\label{sec:simulation}
%In this section, we test models' ability in capturing complex graph filters on 2d-grid data generated by 3 simulation operations:
To compare the representation power of DSGC and GC (given comparable number of parameters), we generated simulated data for the following tasks:
\begin{itemize}
\item \textbf{Shift}: Shift the input graph 1 step to the right. 
\item \textbf{Rotation}: Rotate the input graph by 90 degree. 
\item \textbf{Flip}: Left-Right flip the input graph.
\end{itemize}
Toy examples for those tasks are visualized in Figure \ref{fig:sim}.

We use identical hyper-parameter settings for DSGC- and GC-based architectures in all those tasks, including the number of layers (fixed to be 3) and the activation function. The total numbers of model parameters of DSGC and GC are roughly equal.

The training loss curves for GC and DSGC are shown in Figure \ref{fig:sim-result}, where DSGC clearly outperforms GC.
This is because GC treats the surrounding nodes for any given node as exchangeable \citep{nips2017geo},
while DSGC learns to distinguish the neighbors conditioned on the tasks.
The ability of learning asymmetric relationships is important in real applications such as wind power forecasting because of the directional influences (trends and anisotropy) from one geographic location to its adjacent locations.

% This feature limits its ability to model the propagation pattern. For example, if the input data is a symmetric matrix, the output is also symmetric.

% This is because GC to fail is that the spectral kernel of GC is isotropic due to the rotation invariant of the Laplacian filter \citep{nips2017geo}.

% Moreover, GC cannot capture the asymmetric operations in this simulation experiment. If we predefine specific graph filter for GC for each simulation operation, it can learn the simulation operations. But it still cannot model 3 operations simultaneously with a fixed graph filter. And the DSGC can capture all patterns by learning multiple graph filters. 

% This simulation test shows the flexible graph filter is necessary to capture complex propagation patterns in the data. 



==> table/dataset.tex <==
\begin{table}
\centering
\begin{tabular}{c|cccc}
\hline
Dataset & N & T & Time Interval & Type\\
\hline
TMAX	& 1,218 & 32,507 & 1 day 	& daily maximum temperature	\\
%USHCN-TMIN	& 1,218 & 32,507 & 1 day 	& daily minimum temperature	\\
PRCP	& 1,218 & 32,507 & 1 day	& daily precipitation \\
Solar		& 1,082 & 52,560 & 10 mins 	& energy output of solar plants\\
%Traffic		& 862	& 50,688 & 10 mins 	& traffic usage\\
\hline
\end{tabular}
\caption{Data Statistics of spatiotemporal regression task. N is the number of sensors, T is the number of time stamps, Interval means the time length between two consecutive time stamps.}
\label{tab:dataset}
\end{table}
